Disentangling the composite continuum of symbiotic binaries I. S-type systems

We describe a method of disentangling the composite,0.12-5 microns continuum of symbiotic binaries.The observed SED is determined by the IUE/HST archival spectra and flux-points corresponding to the optical UBVRI and infrared JHKLM photometric measurements. The modeled SED is given by superposition of fluxes from the cool giant, hot stellar source and nebula including the effect of the Rayleigh scattering process and considering influence of the iron curtain absorptions.We applied this method to 21 S-type symbiotic stars during quiescence, activity and eclipses.

==> objects <==
\SIMBADobj{EG And}
\SIMBADobj{Z And}
\SIMBADobj{AE Ara}
\SIMBADobj{CD-43 14304}
\SIMBADobj{TX CVn}
\SIMBADobj{T CrB}
\SIMBADobj{BF Cyg}
\SIMBADobj{CH Cyg}
\SIMBADobj{CI Cyg}
\SIMBADobj{V1329 Cyg}
\SIMBADobj{LT Del}
\SIMBADobj{AG Dra}
\SIMBADobj{CQ Dra}
\SIMBADobj{V443 Her}
\SIMBADobj{YY Her}
\SIMBADobj{RW Hya}
\SIMBADobj{SY Mus}
\SIMBADobj{AR Pav}
\SIMBADobj{AG Peg}
\SIMBADobj{AX Per}
\SIMBADobj{BD-21 3873}
\SIMBADobj{MWC 560}

